A Survey of Multi-task Learning in Natural Language Processing: Regarding Task Relatedness and Training Methods

Multi-task learning (MTL) has become increasingly popular in natural language processing (NLP) because it improves the performance of related tasks by exploiting their commonalities and differences. Nevertheless, it is still not understood very well how multi-task learning can be implemented based on the relatedness of training tasks. In this survey, we review recent advances of multi-task learning methods in NLP, with the aim of summarizing them into two general multi-task training methods based on their task relatedness: (i) joint training and (ii) multi-step training. We present examples in various NLP downstream applications, summarize the task relationships and discuss future directions of this promising topic.

==> 2related.tex <==
Multi-task learning (MTL) is a subfield of machine learning. It aims to leverage useful information shared across multiple related tasks to improve the generalization performance on all the tasks~\cite{caruana1997multitask}. 
% MTL improves generalization by leveraging the domain-specific information contained in the training signals of related tasks.
In recent years, MTL has led to great successes across various applications of machine learning such as natural language processing and computer vision~\cite{ruder2017overview}.

We reviewed relevant surveys published in recent years.
\citet{ruder2017overview} classified different MTL frameworks into two categories: hard parameter sharing and soft parameter sharing, as well as some earlier MTL examples in both non-neural and neural models.
% In hard parameter sharing, all tasks share the same hidden layers, while keeping several task-specific output layers.
% In soft parameter sharing, each task has its own model and parameters.
% The distance between the parameters of the model is then regularized in order to encourage the parameters to be similar. 
\citet{zhang2018overview} expanded such two ``how to share'' categories into five categories, including feature learning approach, low-rank approach, task clustering approach, task relation learning approach, and decomposition approach, and then discussed the characteristics of each approach. 
\citet{worsham2020multi} summarized multi-task learning in NLP from the perspective of when to use multi-task learning and how to use multi-task learning.

{\citet{ruder2017overview} and \citet{crawshaw2020multi} also reviewed detailed techniques of MTL model frameworks. Different from their surveys, our motivation lies in categorizing two major multi-task training methods in NLP, according to task relatedness. With specific application tasks, readers are able to identify the ideal training method from our review before looking for detailed module implementation in previous surveys. We also show that how the MTL techniques covered in previous surveys can be categorized into the two training methods in Table \ref{tab:frameworks}.}



% \citet{ruder2017overview} and \citet{crawshaw2020multi} also gave more fine-grained categories of MTL frameworks based on parameter sharing designs, as shown in Table \ref{tab:frameworks}.
% Different from the motivation of their works, our classification criteria focus on task dependency and information flow in multi-task learning frameworks. We present a guide of choosing coarse-grained frameworks according to model relatedness, while fine-grained model details, such as selecting the parameter sharing technique, can be referred to previous surveys. Table \ref{tab:frameworks} illustrates how existing categories of MTL frameworks are merged into our joint training or multi-step training. Besides, our review is more focused on NLP tasks and applications.



==> 8useKG.tex <==
Previous sections introduced different NLP tasks that are simultaneously trained for better performance, as well as the relatedness between these tasks, which elicit the concepts of nodes and edges in our MTKG.
In this section, we formally denote the multi-task architecture graph (MTAG) and MTKG. We then present an algorithm that can automatically design a \emph{potentially effective} architecture for multi-task training, given any set of NLP tasks.

%\vspace{-0.05in}
\subsection{Notations}

MTAG is used for representing the architecture of multi-task models, in which nodes are encoder/decoder modules and edges are relationships between these modules, \textit{i.e.}, information passing or parameter sharing:

\begin{definition}[Multi-task Architecture Graph]
Suppose we have $n$ tasks.
We denote the MTAG by $G_{arch}=(\mathcal{E}, \mathcal{D}; \mathcal{R}_{pass}, \mathcal{R}_{share})$ where $\mathcal{E}=\{E_1, \dots, E_n\}$ is the set of encoders for the tasks, $\mathcal{D}=\{D_1, \dots, D_n\}$ is the set of decoders, $\mathcal{R}_{pass} \subset {(\mathcal{E} \cup \mathcal{D})}^2$ represents the set of information-passing connections between encoder/decoder modules, and $\mathcal{R}_{share} \subset {\mathcal{E}}^2 \cup {\mathcal{D}}^2$ denotes the parameter-sharing relationship. Note that $\mathcal{R}_{share}$ is symmetric.
\end{definition}

% \begin{figure}[h]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/framework-basic.pdf}
% \caption{Two types of basic encoder-decoder architectures (dashed blocks) for multi-task training.}
% \label{fig:framework-basic}
% \end{figure}

For the two typical MTL frameworks, their architecture graph (AG) can be specified as:

\begin{definition}[Joint training AG]
It is a multi-task architecture graph where
\begin{compactitem}
\item $\mathcal{R}_{pass} = \cup_{i=1}^n \{(E_i, D_i)\}$: information is separately passed from the encoder to decoder on each task;
\item $\mathcal{R}_{share} \approx \cup_{i \neq j} \{(E_i, E_j), (D_i, D_j)\}$: model parameters are \emph{often} shared (in hard or soft ways \cite{ruder2017overview}) among encoders and among decoders so that the tasks can be jointly trained, as shown in Figure~\ref{fig:frameworks-basic}(a). Some missing sharing behavior is allowed.
\end{compactitem}
\end{definition}

\begin{definition}[Multi-step AG]
It is a multi-task architecture graph where
\begin{compactitem}
\item $\mathcal{R}_{pass} \supset \cup_{i=2}^{n} \{(D_{i-1}, D_i)\}$: For task $i$, the input of decoder $D_i$ contains the output or hidden representation of previous decoder $D_{i-1}$;
\item $\mathcal{R}_{share} \approx \cup_{i \neq j} \{(E_i, E_j)\}$: Usually, parameter sharing only appears in encoders; the decoders would no longer share parameters but directly transmit information. 
% See Figure~\ref{fig:frameworks-basic}(b) for example.
\end{compactitem}
\end{definition}

MTKG summarizes the task relatedness in previous MTL researches, in which nodes are different NLP tasks and edges are knowledge transfer directions used by previous approaches:

\begin{definition}[Multi-task Knowledge Graph]
We denote the MTKG by $G_{MTK}=(\mathcal{T}; \mathcal{R}_{trans};$ $ w_{trans}, w_{share-E},$ $w_{share-D})$, where $\mathcal{T}$ is the set of NLP tasks, $\mathcal{R}_{trans} \in \mathcal{T}\times\mathcal{T}$ has directed edges from one task to another if there was at least one existing study that performed knowledge transfer to train model(s) on the two tasks. If two tasks can be jointly trained, then we connect them with a bi-directional edge. Each edge has three weighting functions in the form of $w: \mathcal{R}_{trans} \rightarrow {\mathbb{Z}}^+$, denoting the number of methods that considered the transfer, encoder parameter sharing, and decoder parameter sharing, respectively.
\end{definition}

Given the above definitions, We constructed MTKG-1.0, based on 141 multi-task learning NLP papers collected from top AI/NLP conferences and journals, \textit{e.g.}, AAAI, ACL, ICLR, TACL, etc. MTKG-1.0 consists of 56 nodes (tasks) and 213 edges, with a subgraph shown in Figure \ref{fig:mtkg}. 
% We put more descriptions, statistics, and a visualization system for MTKG-1.0 at the following repository \url{https://github.com/wyu97/MTKG}.

MTKG connects a variety of tasks across different NLP domains, which displays what tasks are involved in MTL previously and implicitly expresses task relatedness. Based on these features of MTKG, in this work, we are interested in automatically designing a potentially effective model architecture for a set of specific NLP tasks using MTKG. Such architecture prediction can serve as preliminary attempts when researchers are faced with a set of different NLP tasks that have not been simultaneously trained before. Thus we have:

% \begin{problem}[Tasks-specified MTAG Design]
% Given a set of tasks $\mathcal{T}_{spec} \subset \mathcal{T}$ (along with training data), our goal is to find a potentially successful multi-task training architecture $G_{arch}$.
% \end{problem}
\begin{problem}[Tasks-specified MTAG Design]
Given a set of tasks $\mathcal{T}_{spec} \subset \mathcal{T}$, find a potentially successful multi-task training architecture $G_{arch}$.
\end{problem}



% \subsection{Problem}

% Datasets for a variety of tasks can be collected in many NLP domains.
% For example, named entity recognition, summarization, reading comprehension, and question answering are important tasks for legal techs.
% Building an effective learning architecture needs expertise and skills of a research team. We are interested in automatically designing an architecture for a set of specific NLP tasks.  

% \begin{problem}[Tasks-specified MTAG Design]
% Given a set of tasks $\mathcal{T}_{spec} \subset \mathcal{T}$ (along with training data), our goal is to find a potentially successful multi-task training architecture $G_{arch}$.
% \end{problem}

\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/autoag.pdf}
%\vspace{-0.2in}
\caption{Auto-designing a multi-task architecture graph (MTAG) from specified tasks using our multi-task knowledge graph (MTKG).}
%\vspace{-0.1in}
\label{fig:autoag}
\end{figure}


%\vspace{-0.05in}
\subsection{Algorithm}

The algorithm of automatically designing a MTL framework has three steps as follows.

% %\vspace{-0.05in}
\paragraph{Step 1: Find necessary additional tasks.}

If tasks in $T_{spec}$ are already connected in $G_{MTK}$, then we can directly perform multi-task learning on these tasks. Otherwise, we need to find the minimal number of additional tasks $T_{add}$ that can maximize the number of connected tasks. As in Figure \ref{fig:autoag}, $T_{add} = \{T_5\}$.
The nodes in the new subgraph should be $\mathcal{T}_{spec} \cup \mathcal{T}_{add}$.
Then the number of tasks considered in our MTL framework is $n = |\mathcal{T}_{spec} \cup \mathcal{T}_{add}|$. So we have the set of encoders $\mathcal{E}$ and the set of decoders $\mathcal{D}$, each of size $n$.

%Initialize the set of additional tasks needed as $\mathcal{T}_{add} = \{\}$.
%  The first step is to find the minimal number of additional tasks that can be used to perform MTL. For each task $T$, we find the shortest paths between $T$ and other task $T' \in \mathcal{T}_{spec}$ on $G_{MTK}$.
% Search the minimum number of additional (task) nodes $|\mathcal{T}_{add}|$ that can maximize the number of connected components of the subgraph formed by the set of nodes $\mathcal{T}_{spec} \cup \mathcal{T}_{add}$ on $G_{MTK}$.
% % Choose the path of the smallest length and add the tasks on the path that are not included in $\mathcal{T}_{spec}$ into $\mathcal{T}_{add}$.
% Then the number of tasks in the AG is $n = |\mathcal{T}_{spec} \cup \mathcal{T}_{add}|$. So we have the set of encoders $\mathcal{E}$ and the set of decoders $\mathcal{D}$, each of size $n$.

% %\vspace{-0.05in}
\paragraph{Step 2: Determine directions of knowledge transfer.}
Encoder-decoder models usually use the hidden representations of the encoder as the input of the decoder. Thus, we initialize the information-passing set $\mathcal{R}_{pass}$ with the encoder $\rightarrow$ decoder edges, \textit{i.e.}, $\mathcal{R}_{pass} = \cup_{i=1}^n \{(E_i, D_i)\}$. For a pair of tasks $T_i$ and $T_j$, if there exists a uni-directional edge between them on $G_{MTK}$, \textit{i.e.}, $(T_i, T_j) \in \mathcal{R}_{trans}$ and $(T_j, T_i) \notin \mathcal{R}_{trans}$, then knowledge should be transferred from the decoder of $T_i$ to that of $T_j$, \textit{i.e.}, $\mathcal{R}_{pass}\leftarrow\mathcal{R}_{pass} \cup \{(D_i, D_j)\}$. Given the example in Figure~\ref{fig:autoag}, the knowledge transfer direction among decoders in $G_{arch}$ should be $D_2 \shortrightarrow D_5 \shortrightarrow D_4 \shortrightarrow D_3$.

% %\vspace{-0.05in}
\paragraph{Step 3: Determine strategies of parameter sharing}
Initialize $\mathcal{R}_{share} = \varnothing$. We suggest to share the parameters between encoders/decoders when there were more existing studies that suggested parameter sharing than those that did not. Specifically, for encoders, if the edge $(T_i,T_j)$ satisfies $w_{share-E}(T_i, T_j) > w_{trans}(T_i, T_j)/2$, then we share the encoders of task $T_i$ and $T_j$, namely $\mathcal{R}_{share} \leftarrow \mathcal{R}_{share} \cup \{(E_i, E_j)\}$. However, for decoders, parameter sharing usually appear in joint training, which requires a bi-directional edge between two tasks. Thus, if both $(T_i, T_j)$ and $(T_j, T_i) \in \mathcal{R}_{trans}$, and $w_{share-D}(T_i, T_j)>w_{trans}(T_i, T_j)/2$, then we share their decoders, namely $\mathcal{R}_{share} \leftarrow \mathcal{R}_{share} \cup \{(D_i, D_j)\}$. For instance, in Figure~\ref{fig:autoag} we have $(E_1, E_2), (E_3, E_4), (E_4, E_5), (E_3, E_5)$ and $(D_1, D_2)$ in $\mathcal{R}_{share}$ due to the numerical relationships of the corresponding weighting functions. We recommend to collect training data for $T_5$ and then use the above architecture to train a multi-task learning model on the five NLP tasks.


% For a pair of tasks $T_i$ and $T_j$, when both $(T_i, T_j)$ and $(T_j, T_i) \in \mathcal{R}_{trans}$, if $w_{share-E}(T_i, T_j) > w_{trans}(T_i, T_j)/2$, then we share their encoders, $\mathcal{R}_{share} \leftarrow \mathcal{R}_{share} \cup \{(E_i, E_j)\}$; if $w_{share-D}(T_i, T_j)>w_{trans}(T_i, T_j)/2$, then we share their decoders, $\mathcal{R}_{share} \leftarrow \mathcal{R}_{share} \cup \{(D_i, D_j)\}$. That is, we suggest to share the parameters between encoders/decoders when there were more existing studies that suggested parameter sharing than those that did not. In Figure~\ref{fig:autoag}, %because there was a joint training AG of $T_1$ and $T_2$, and a multi-step AG of $T_5$, $T_4$, and $T_3$, 
% considering the weights of the edges, we have (a) $(E_1, E_2), (E_3, E_4), (E_4, E_5), (E_3, E_5)$ and (b) $(D_1, D_2)$ in $\mathcal{R}_{share}$. Therefore, we recommend to collect training data for $T_5$ and then use the above architecture to train a model on the five NLP tasks.


==> tables/table_layers.tex <==
% \begin{table}[t]
% \begin{center}
% \scale[0.85]{\begin{tabular}{|l|l|}
% \hline
% \multicolumn{2}{|l|}{\textbf{Embedding Layer:}} \\ \hline
% TokenEmb & Token embedding \\ \hline
% CharEmb & Character embedding \\ \hline
% PosEmb & Position embedding \\ \hline
% EntEmb & Entity embedding \\ \hline
% \hline
% \multicolumn{2}{|l|}{\textbf{Encoder Layer:}} \\ \hline
% GRU & Gated recurrent units \\ \hline
% BiLSTM & Bidirectional Long Short-Term Memory \\ \hline
% % & Memory networks \\ \hline
% Attention & Attention mechanism \\ \hline
% Iteration & Iteration mechanism \\ \hline
% Transformer & Multi-head self-attention \\ \hline % model
% % BERT & Bidirectional encoder representations \\
% % & from Transformers \\ \hline
% CNN & Convolutional neural networks \\ \hline
% GCN & Graph convolutional networks \\ \hline
% \hline
% \multicolumn{2}{|l|}{\textbf{Decoder Layer:}} \\ \hline
% FFNN & Feed-forward neural networks \\ \hline
% LSTM & Long Short-Term Memory networks \\ \hline
% CRF & Conditional random fields \\ \hline
% CapsNet & Capsule neural network \\ \hline
% LR & Logistic regression \\ \hline
% % Softmax & Softmax function \\ \hline
% Transformer & Multi-head self-attention \\ \hline
% \hline
% \multicolumn{2}{|l|}{\textbf{Optimization:}} \\ \hline
% MinSumLoss & Minimize sum of cross-entropy losses \\ \hline
% MaxJointLH & Maximize joint likelihood \\ \hline
% RL & Reinforcement learning \\ \hline
% \end{tabular}}
% \end{center}
% \vspace{-0.1in}
% \caption{Choices of modules in each layer of the frameworks. One or multiple choices are allowed.}
% \label{tab:layers}
% \vspace{-0.1in}
% \end{table}


==> tables/table_slu_modules.tex <==
% \begin{table*}[t]
% \begin{center}
% \scale[0.9]{\begin{tabular}{|l|l|l|l|l|l|}
% \cline{2-6}
% \multicolumn{1}{l|}{} & \textbf{Embedding Layer} & \textbf{Encoder Layer} & \multicolumn{2}{|l|}{\textbf{Decoder Layer}} & \textbf{Optimization} \\ \cline{4-5}
% \multicolumn{1}{l|}{} & & & \textbf{SF} & \textbf{ID} & \\ \hline
% \cite{xu2013convolutional} & TokenEmb & n/a & CRF & CNN & MaxJointLH \\ \hline
% \cite{zhang2016joint} & TokenEmb, \underline{EntEmb} & GRU & SoftMax & Softmax & MinSumLoss \\ \hline
% \cite{liu2016attention} & TokenEmb & \underline{BiLSTM} & LR & LR & n/a \\ \hline
% \cite{goo2018slot} & n/a & BiLSTM, \underline{Attention} & Softmax & Softmax & MaxJointLH \\ \hline
% \cite{yu2018acjis} & n/a & BiLSTM, \underline{Attention} & \underline{CRF} & \underline{CRF} & MinSumLoss \\ \hline
% \cite{haihong2019novel} & n/a & BiLSTM, \underline{Iteration} & CRF & Softmax & n/a \\ \hline
% \cite{zhang2019joint} & n/a & BiLSTM & \underline{CapsNet} & \underline{CapsNet} & MinSumLoss \\ \hline
% \cite{castellucci2019multi} & n/a & \underline{BERT} & Softmax & Softmax & MinSumLoss \\ \hline
% \cite{chen2019bert} & TokenEmb, PosEmb & \underline{BERT} & \underline{CRF} & Softmax & MinSumLoss \\ \hline
% \end{tabular}}
% \end{center}
% \vspace{-0.1in}
% \caption{Joint training techniques for multi-task SLU and their modules of the four components. The underlined modules are for the technical novelty. SF is for slot filling. ID is for intent detection.}
% \label{tab:slu_modules}
% \end{table*}


==> tables/table_slu_results.tex <==
\begin{table*}[t]
\begin{center}
\scale[0.85]{\begin{tabular}{|l|l|l|l|c|c|c|c|}
\cline{2-8}
\multicolumn{1}{l|}{\textbf{}} & \multicolumn{1}{l|}{\textbf{Encoder}} & \multicolumn{2}{c|}{\textbf{Decoder}} & \multicolumn{2}{c|}{\textbf{ATIS}} & \multicolumn{2}{c|}{\textbf{SNIPS}} \\ \cline{3-8}
\multicolumn{1}{l|}{\textbf{}} & \multicolumn{1}{l|}{\textbf{}} & SF & ID & SF (F1) & ID (Acc.) & SF (F1) & ID (Acc.) \\ \hline
\cite{goo2018slot} & BiLSTM & FFNN & FFNN & 95.2 & 94.1 & 88.8 & 97.0 \\ \hline
\cite{zhang2019joint} & BiLSTM & CapsNet & CapsNet & 95.2 & 95.0 & 91.8 & 97.3 \\ \hline
\cite{haihong2019novel} & BiLSTM & CRF & FFNN & 95.8 & 97.1 & 91.4 & 97.4 \\ \hline
\cite{castellucci2019multi} & BERT & FFNN & FFNN & 95.7 & 97.8 & 96.2 & \textbf{99.0} \\ \hline
\cite{chen2019bert} & BERT & CRF & FFNN & \textbf{96.0} & \textbf{97.9} & \textbf{97.0} & 98.6 \\ \hline
\end{tabular}}
\end{center}
\vspace{-0.1in}
\caption{The performance of multi-task SLU techniques on ATIS and SNIPS benchmark datasets.}
\label{tab:slu_results}
\end{table*}


==> tables/table_tasks.tex <==
% \begin{table*}[t]
% \begin{center}
% \scale[0.85]{\begin{tabular}{|l|l|l|l|}
% \hline
% \multicolumn{2}{|l|}{\textbf{NLP Task}} & \textbf{Input} & \textbf{Output} \\ \hline
% \hline
% IE & Information Extraction & Texts & Structured forms of information \\ \hline
% NER & Named Entity Recognition & Sentence / Token & \{Named entities\} / Entity tag \\ \hline
% RE & Relation Extraction & Sentence & \{(Entity$_1$, Entity$_2$, Relation)\} \\ \hline % / Token / Relation tag
% \hline
% SLU & Spoken Language Understanding & Spoken or written language & Meaning of human language \\ \hline
% SF & Slot Filling & Token & Label \\ \hline
% ID & Intent Detection & Sentence & Intent \\ \hline
% \hline
% NLG & Natural language generation & Texts, image, graph and etc & Natural language text \\ \hline
% MT & Neural Translation & Text sequence & Text sequence \\ \hline
% AS & Abstractive summarization & Text document & Text sequence \\ \hline
% DS & Dialogue system & Text sequence & Text sequence \\ \hline
% QG & Question generation & Answer & Question \\ \hline
% CR & Creative writing & Text sequence & Text sequence \\ \hline
% \hline
% MPQA & Multi-Passage Question Answering & Question, \{Passages\}, (\{Answers\}) & Best answer \\ \hline
% PR & Passage Retrieval & Question, \{Passages\} & \{Relevant passages\} \\ \hline
% RC & Reading Comprehension & Question, Relevant passage & Answer span \\ \hline
% AR & Answer Reranking & \{Answer spans\} & Best answer \\ \hline
% GR & Graph-based Reasoning & Question, Passage graph & Path \\ \hline
% PS & Path/answer Selection & \{Paths (answers)\} & Best path (answer) \\ \hline
% \end{tabular}}
% \end{center}
% \vspace{-0.1in}
% \caption{Acronym, full name, and description of typical NLP applications discussed in this paper.}
% \label{tab:tasks}
% \end{table*}

